Covert Computation in Self-Assembled Circuits

Traditionally, computation within self-assembly models is hard to conceal because the self-assembly process generates a crystalline assembly whose computational history is inherently part of the structure itself. With no way to remove information from the computation, this computational model offers a unique problem: how can computational input and computation be hidden while still computing and reporting the final output? Designing such systems is inherently motivated by privacy concerns in biomedical computing and applications in cryptography. In this paper we propose the problem of performing ``covert computation'' within tile self-assembly that seeks to design self-assembly systems that ``conceal'' both the input and computational history of performed computations. We achieve these results within the growth-only restricted abstract Tile Assembly Model (aTAM) with positive and negative interactions. We show that general-case covert computation is possible by implementing a set of basic covert logic gates capable of simulating any circuit (functionally complete). To further motivate the study of covert computation, we apply our new framework to resolve an outstanding complexity question; we use our covert circuitry to show that the unique assembly verification problem within the growth-only aTAM with negative interactions is coNP-complete.

==> properties.tex <==

\section{Formal Definitions} \label{app:def}

\textbf{Tiles.}
Let $\Pi$ be an alphabet of symbols called the \emph{glue types}.  A tile is a finite edge polygon with some finite subset of border points each assigned a glue type from $\Pi$.  Each glue type $g \in \Pi$ also has some integer strength $str(g)$.
Here, we consider unit square tiles of the same orientation with at most one glue type per face, and the \emph{location} to be the center of the  tile  located at integer coordinates.




\textbf{Assemblies.}
An assembly is a finite set of tiles whose interiors do not overlap.  %Further, to simplify formalization in this paper, we require the center of each tile in an assembly to be an integer coordinate.
If each tile in $A$ is a translation of some tile in a set of tiles $T$, we say that $A$ is an assembly over tile set $T$.   For a given assembly $\Upsilon$, define the \emph{bond graph} $G_\Upsilon$ to be the weighted graph in which each element of $\Upsilon$ is a vertex, and the weight of an edge between two tiles is the strength of the overlapping matching glue points between the two tiles.  Only overlapping glues of the same type contribute a non-zero weight, whereas overlapping, non-equal glues  contribute zero weight to the bond graph.  The property that only equal glue types interact with each other is referred to as the \emph{diagonal glue function} property and is perhaps more feasible than more general glue functions for experimental implementation (see~\cite{AGKS05g} for the theoretical impact of relaxing this constraint).  An assembly $\Upsilon$ is said to be \emph{$\tau$-stable} for an integer $\tau$ if the min-cut of $G_\Upsilon$ is at least $\tau$.

\textbf{Tile Attachment.}
Given a tile $t$, an integer $\tau$, and an assembly $A$, we say that $t$ may attach to $A$ at temperature $\tau$ to form $A'$ if there exists a translation $t'$ of $t$ such that $A' = A \bigcup \{t'\}$, and the sum of newly bonded glues between $t'$ and $A$ meets or exceeds $\tau$.  For a tile set $T$ we use notation $A \rightarrow_{T,\tau} A'$ to denote  there exists some $t\in T$ that may attach to $A$ to form $A'$ at temperature $\tau$.  When $T$ and $\tau$ are implied, we simply say $A \rightarrow A'$.  Further, we say that $A \rightarrow^*A'$ if either $A=A'$, or there exists a finite sequence of assemblies $\langle A_1 \ldots A_k\rangle$ such that $A \rightarrow A_1 \rightarrow \ldots \rightarrow A_k \rightarrow A'$.

\textbf{Tile Systems.}
A tile system $\Gamma = (T,S, \tau)$ is an ordered triplet consisting of a set of tiles $T$ called the system's \emph{tile set}, a $\tau$-stable assembly $S$ called the system's \emph{seed} assembly, and a positive integer $\tau$ referred to as the system's \emph{temperature}. A tile system $\Gamma = (T,S,\tau)$ has an associated set of \emph{producible} assemblies, $\texttt{PROD}_\Gamma$, which define what assemblies can grow from the initial seed $S$ by any sequence of temperature $\tau$ tile attachments from $T$.  Formally, $S \in \texttt{PROD}_\Gamma$ is a base case producible assembly.  Further, for every $A\in \texttt{PROD}_\Gamma$, if $A \rightarrow_{T,\tau} A'$, then $A' \in \texttt{PROD}_\Gamma$.  That is, assembly $S$ is producible, and for every producible assembly $A$, if $A$ can grow into $A'$, then $A'$ is also producible.  %In other words, the set of producible assemblies contains any assembly that can be obtained by any valid sequence of tile attachments starting from assembly $S$.
We further denote a producible assembly $A$ to be \emph{terminal} if $A$ has no attachable tile from $T$ at temperature $\tau$.  We say a system $\Gamma=(T,S,\tau)$ \emph{uniquely produces} an assembly $A$ if all producible assemblies can grow into $A$ through some sequence of tile attachments.  More formally, $\Gamma$ \emph{uniquely produces} an assembly $A \in \texttt{PROD}_\Gamma$ if for every $A' \in \texttt{PROD}_\Gamma$ it is the case that $A' \rightarrow^* A$.  Systems that uniquely produce one assembly are said to be \emph{deterministic}. 

Finally, we consider a system to be a \emph{valid growth-only} system if all assemblies in $\texttt{PROD}_\Gamma$ are $\tau$-stable. The existence of negative strength glues allows for the possibility that unstable assemblies are produced. %Unique Assembly Verification is undecidable when unstable assemblies are allowed. 
%Thus, in this paper we restrict our consideration to valid growth-only systems.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Gadget Properties} \label{app:props}

Here, we describe some of the gadgets in more detail by specifying the properties that each gadget must have in order to guarantee covert operation.

\subsection{Logic Diodes} \label{subapp:logic}

Logic Diodes are important to prevent timing issues in the dual rail logic related to backfilling of the covert gadgets. They must have these properties.
\begin{itemize}
    \item[\textbf{1.}] If $t_i^{in}$ enters, then only $t_i^{out}$ leaves. This is guaranteed due to $h_2,h_3$ cooperatively placing the next tile. Without $f_i^{in}$ present, the only next tile which could be placed is this cooperatively-placed tile from $t_i^{out}$.
    \item[\textbf{2.}] If $f_i^{in}$ enters, then only $f_i^{out}$ leaves. This is guaranteed due to $h_4,h_5$ cooperatively placing the next tile. Without $t_i^{in}$ present, the only next tile which could be placed is this cooperatively-placed tile from $f_i^{out}$.
    \item[\textbf{3.}] The $f_i^{in}$ wire will be backfilled if and only if $t_i^{in}$ enters. Without $t_i^{in}$ present, a given backfilled false path will stop at the tile with $h_4,h_5$. With $t_i^{in}$ present, the tile with $h_1,h_4$ can cooperatively attach and backfill the false wire.

    %\item[\textbf{C3.}] If $t_i^{in}$ enters, and the gadget backfills the false path, then the $f_i^{in}$ wire will be backfilled. Given a backfilled false path it will stop at the tile with $h_4,h_5$. However, since the true wire is there, the tile with $h_1,h_4$ can cooperatively attach and backfill the false wire.
    \item[\textbf{4.}] The $t_i^{in}$ wire will be backfilled if and only if $f_i^{in}$ enters. Without $f_i^{in}$ present, a backfilled false path will stop at the tile with $h_2,h_3$. However, with $f_i^{in}$ present, the $h_1,h_2$ tile  can cooperatively attach and backfill the false wire.
    %\item[\textbf{C4.}] If $f_i^{in}$ enters, and the gadget backfills the false path, then the $t_i^{in}$ wire will be backfilled. Given a backfilled true path it will stop at the tile with $h_2,h_3$. However, since the false wire is there, the tile with $h_1,h_2$ can cooperatively attach and backfill the true wire.
\end{itemize}

\subsection{NOT Gadget} \label{subapp:NOT}
In verifying that the gadget works as intended, we must verify six properties.
\begin{itemize}
    \item[\textbf{1.}] If $t_i^{in}$ enters a NOT gadget, it results in $f_i^{out}$ and not $t_i^{out}$.
    Figure \ref{fig:ccnott1} shows the gadget in this case$-$ with true input $t_i^{in}$ and output $f_i^{out}$. The true output can not place from tile $x$ due to the negative glues $n_1$ and $n_3$ of strength $-1$. Given the build order, we are guaranteed $f_i^{out}$ and that $t_i^{out}$ can not build.

    \item[\textbf{2.}] If $f_i^{in}$ enters a NOT gadget, it results in $t_i^{out}$ and not $f_i^{out}$.
    Figure \ref{fig:ccnotf1} shows the gadget in this case$-$ with false input $f_i^{in}$ and output $t_i^{out}$. The false output can not attach due to the negative glue $n_2$. The tile to the west of $x$ may attach, but due to glue $n_3$, no other tile can attach. Given the build order, we are guaranteed $t_i^{out}$ and that $f_i^{out}$ can not build.

    \item[\textbf{3.}] If $t_i^{in}$ enters a NOT gadget and $f_i^{out}$ leaves, the gadget and $f_i^{in}$ is backfilled up to tile $x$. Figure \ref{fig:ccnott2} shows the desired result. Glues $h_3,h_4$ cooperatively allow the false portion and wire to backfill. Glue $h_2$ is needed to fill in the tile with $n_2$.

    \item[\textbf{4.}] If $f_i^{in}$ enters a NOT gadget and $t_i^{out}$ leaves, the gadget and $t_i^{in}$ is backfilled up to tile $x$. Figure \ref{fig:ccnotf2} shows the desired result. Glues $h_5,h_6$ allow the true portion and wire to backfill. Glue $h_1$ is needed to counteract the $n_1$ glue when backfilling that tile.

    \item[\textbf{5.}] If the gadget resulted in $f_i^{out}$, a future gadget can backfill $t_i^{out}$ and the gadget will be complete. If the gadget is in the configuration of Figure \ref{fig:ccnott2}, the true wire can directly backfill until the tile directly above tile $x$. The glue $n_1$ would prevent this tile from placing except $x$ will be there and the tile can cooperatively be placed using the north glue of $x$ and the south glue of the backfilling wire.

    \item[\textbf{6.}] If the gadget resulted in $t_i^{out}$, a future gadget can backfill $f_i^{out}$ and the gadget will be complete. If the gadget is in the configuration of Figure \ref{fig:ccnotf2}, the false wire can directly backfill until the tile directly east of tile $x$. The glue $n_2$ would prevent this tile from placing except $x$ is there and the tile can cooperatively be placed using the east glue of $x$ and the west glue of the backfilling wire.
\end{itemize}

The first two conditions guarantee that the gadget works correctly. The second two conditions guarantee the covertness of the gadget, i.e., the gadget looks indistinguishable before the output regardless of the input. The final two conditions verify that the backfill from future gadgets will work correctly, and no trace of the build path will be evident.



\subsection{NAND Gadget} \label{subapp:NAND}

%For clarity, we show that the NAND works with the block diagram first, then address a few technical issues in the full version. We need to verify the following.
There are many specific issues related to the NAND gadget handled in the text. The properties that it must have are as follows.
\begin{itemize}
    \item[\textbf{1.}] Given $f_i^{in}$ or $f_j^{in}$, the wire $t_{ij}^{out}$ leaves the gadget. If wire $f_i^{in} = t_i^{out}$ is set, this is tied directly to the output wire $t_{ij}^{out}$. If the wire $f_j^{in}$ comes in, it comes in as the false input of the second H-NOT gadget, which means it leaves as $t_{ij}^{out}$ by the validity of the NOT gadget.

    \item[\textbf{2.}] If wires $t_i^{in}$ and $t_j^{in}$ are set, then the wire $f_{ij}^{out}$ should leave the gadget. Wire $t_i^{in}$ exits the first NOT gadget as $f_i^{out}$. This wire, $f_i^{out}$, and $t_j^{in}$ both stop and expose glues $a_2$ and $a_3$, respectively. Both are strength 1 glues, and thus the tile with glues $a_2$ and $a_3$ can only place if both the glues are exposed. Thus, only if wires $t_i^{in}$ and $t_j^{in}$ are set, will wire $t_{ij}^{in}$ ever enter the H-NOT gadget, which results in the wire $f_{ij}^{out}$ as the gadget output.

    \item[\textbf{3.}] All components backfill correctly. The NOT gadget backfills correctly. If $f_j^{in}$ was set, then $t_{ij}^{in}$ is backfilled from the H-NOT gate. When the tiles are placed such that glues $a_1$ and $a_2$ are placed, the tile can cooperatively place that backfills $f_i^{out}$. Similarly, when the other tiles place with glues $a_3$ and $a_4$, a tile cooperatively attaches to backfill the $t_j^{in}$.

    \item[\textbf{4.}] The growth-only constraint is not violated with the negative glues. This can only happen given a stable assembly where a tile attaches with a negative glue that destabilizes part of the assembly. The additional negative glue $n_H$ could do this if the green tile is placed after the blue tile, however, the build path is intentional to ensure this can not happen. If the wire $f_{ij}^{out}$ were placed and $t_{ij}^{out}$ is backfilled, the tile with $n_H$ would be the last tile that could attach and the assembly would never be unstable.

    \item[\textbf{5.}] The gadget does not behave incorrectly with only one input. The logic diode guarantees the backfilling never goes beyond the gadget. If one input is false, the NAND can send the $t_{ij}^{out}$ wire and backfill the NAND gadget without having yet receieved the second input. When it arrives, that wire is backfilled.
\end{itemize}

\subsection{FANOUT Gadget} \label{subapp:FANOUT}
The FANOUT gadget needs to duplicate the geometric wire, and also needs to only backfill once both outgoing wires have backfilled. Figure \ref{fig:ccfanout} shows the FANOUT gadget. It has the following necessary properties.

\begin{itemize}
    \item[\textbf{1.}] With input $t_i^{in}$, the gadget outputs wires $t_i^{out_1}$ and $t_i^{out_2}$, and does not output $f_i^{out_1}$ and $f_i^{out_2}$. Figure \ref{fig:fots1} shows the true fanout without the backfilling. Due to $n_1$ and $n_2$, the false outputs can not assemble. Both settings share the same middle four tiles, but with placement order $n_1$ is placed first and then cooperative glues are used to place the first tile of the four (with glues $g_3,g_4$).

    \item[\textbf{2.}] With input $f_i^{in}$, the gadget outputs wires $f_i^{out_1}$ and $f_i^{out_2}$, and does not output $t_i^{out_1}$ and $t_i^{out_2}$. Figure \ref{fig:fofs1} shows the false fanout without the backfilling. Due to $n_1$ and $n_2$, the true outputs can not assemble.  With placement order $n_2$ is placed first and then cooperative glues are used to place the first of the four middle tiles (with glues $h_3,h_4$).

    \item[\textbf{3.}] With input wire $t_i^{in}$, wire $f_i^{in}$ only backfills once $f_i^{out_1}$ or $f_i^{out_2}$ have backfilled. Both wires backfill independently, and only when $f_i^{out_2}$ is backfilled will wire $f_i^{in}$ backfill.

    \item[\textbf{4.}] With input wire $f_i^{in}$, wire $t_i^{in}$ only backfills once $t_i^{out_1}$ or $t_i^{out_2}$ have backfilled. Both wires backfill independently, and only when $t_i^{out_1}$ is backfilled will wire $t_i^{in}$ backfill.
\end{itemize}




